Learning Language Games through Interaction

We introduce a new language learning setting relevant to building adaptive natural language interfaces. It is inspired by Wittgenstein's language games: a human wishes to accomplish some task (e.g., achieving a certain configuration of blocks), but can only communicate with a computer, who performs the actual actions (e.g., removing all red blocks). The computer initially knows nothing about language and therefore must learn it from scratch through interaction, while the human adapts to the computer's capabilities. We created a game in a blocks world and collected interactions from 100 people playing it. First, we analyze the humans' strategies, showing that using compositionality and avoiding synonyms correlates positively with task performance. Second, we compare computer strategies, showing how to quickly learn a semantic parsing model from scratch, and that modeling pragmatics further accelerates learning for successful players.

==> projective.tex <==


\subsection{Projective Parsing}
While the baseline is conceptually simple and makes almost no
assumptions.
Perhaps two constraints are more or less universal here and can be
helpful. Firstly, each formula should be explained projectively. In
this case, projectivity just means that each each node in the tree for
the formula must correspond to a consecutive span in the
utterance. Out of the 6 permutations of {remove, red, block)
  explaining the formula $\text{remove(blocksByColor(red))}$. Two are
  ruled out by this notion of projectivity, where the word to
  predicate correspondence is the obvious one. (red, remove,block),
  (block, remove, red) are not projective.
Second, while a single word can explain multiple predicates, and vice
versa, there should at least be some pressure that if one token is
used to explain a predicate, then it is less likely to explain another
predicate in the formula. And conversely, a token explaining nothing
so far in the search process is more likely to explain a predicate in
the future.

A sample beam parser grammar, with all the freedom, that blows up exponentially.
\begin{lstlisting}[language=lisp]
(rule $A (($P) $X ($P) $Y ($P)))
(rule $A (($P) $Y ($P) $X ($P)))
(rule $B (($P) $Z ($P)))
\end{lstlisting}

\TODO{flesh this out}
\TODO{flesh this out
Write about features
Write about NBest list aggregation
Write about learning
Write about no anchoring, and curriculum.
}

